A Practical Coding Scheme for the BSC with Feedback

We provide a practical implementation of the rubber method of Ahlswede et al. for binary alphabets. The idea is to create the "skeleton" sequence therein via an arithmetic decoder designed for a particular $k$-th order Markov chain. For the stochastic binary symmetric channel, we show that the scheme is nearly optimal in a strong sense for certain parameters.

==> Implementing.tex <==
\section{Implementing Rubber Coding}
